Imitating Human Search Strategies for Assembly

We present a Learning from Demonstration method for teaching robots to perform search strategies imitated from humans in scenarios where alignment tasks fail due to position uncertainty. The method utilizes human demonstrations to learn both a state invariant dynamics model and an exploration distribution that captures the search area covered by the demonstrator. We present two alternative algorithms for computing a search trajectory from the exploration distribution, one based on sampling and another based on deterministic ergodic control. We augment the search trajectory with forces learnt through the dynamics model to enable searching both in force and position domains. An impedance controller with superposed forces is used for reproducing the learnt strategy. We experimentally evaluate the method on a KUKA LWR4+ performing a 2D peg-in-hole and a 3D electricity socket task. Results show that the proposed method can, with only few human demonstrations, learn to complete the search task.

==> Sections/conclusions_prel.tex <==

\section{CONCLUSIONS AND FUTURE WORK}
\label{sec:conclusions}

We presented a simple yet data efficient \ac{lfd} method teaching 
robots to imitate human search strategies for assembly tasks. The key idea is 
to first learn from human demonstrations both an exploration distribution and a 
dynamics 
model and then use these to generate candidate search trajectories covering 
said 
exploration 
distribution with superimposed forces extracted from the dynamics model. We 
evaluated two different trajectory generating methods: \ac{tshix} our own 
sampling based method and ergodic control a deterministic optimal path planner. 
The experimental results demonstrate that our method is data efficient as it 
learns 
to complete 2D and 3D search tasks from only one, respectively, two human 
demonstrations, a major improvement over current exception strategies that have 
been shown to only work in 2D. 

There are several interesting directions for future work. First of all, as we 
observed from demonstrations that humans tend to naturally 
perform 
their search in distinct phases and in no more than three dimensions, it stems 
to 
reason that it is more efficient to model high dimensional searches 
as a sequence of lower-dimensional ones with, \eg, the method presented in 
\cite{hagos2018seq}. Furthermore, as experienced during the initial trials the 
quality of the human demonstrations varied substantially, raising an 
interesting question on how to 
develop teaching environment for both human and robot in order to get high 
quality demonstrations? 

















==> Sections/experiments_prel.tex <==
\section{EXPERIMENTS AND RESULTS}
\label{sec:experiments}
We used a KUKA LWR4+ lightweight arm to experimentally study the method. Demonstrations were recorded in gravity compensation mode, where the robot's internal sensors recorded the pose of the robot and an ATI mini45 \ac{ftsensor} placed at the wrist of the robot recorded the wrench.

We implemented the controller through the Fast Research Interface (FRI)~\cite{schreiber10}, where the controller is defined as
\begin{equation}
  \pmb{\tau}=J^T(\mathrm{diag}(\pmb{k_{FRI}})(\pmb{x^*}-\pmb{x})+\mathrm{diag}(\pmb{d_{FRI}})\pmb{v}+\pmb{F_{FRI}})+\pmb{f_{dyn}}
  \label{eqt:kuka}
\end{equation}
where $\pmb{\tau}$ is the commanded joint torques $J$ is the Jacobian, $\mathrm{diag}(\pmb{k_{FRI}})$ and $\mathrm{diag}(\pmb{d_{FRI}})$ diagonal matrices constructed of the gain and damping values $\pmb{k_{FRI}}$ and $\pmb{d_{FRI}}$, $\pmb{x^*}-\pmb{x}$ the difference between commanded and actual poses and $\pmb{f_{dyn}}$ the feed-forward dynamics. We implemented the controller by setting $\pmb{k_{FRI}}=\pmb{0}$ and feeding the outputs of~\eqref{eq:impedanceControlForce} and~\eqref{eq:impedanceControlTorque} to the superposed Cartesian wrench term $\pmb{F_{FRI}}$.


We evaluated the method in two scenarios, a peg-in-hole task (Fig.~\ref{fig:expSetupPih}) and an electrical plug and socket (Fig.~\ref{fig:expSetupPlug}). With the peg-in-hole setup, we first compared the two presented trajectory creation algorithms, \ac{tshix} and ergodic control. The results of this comparison are shown in Section~\ref{sec:tspVsErgodic}. In Section~\ref{sec:samplingSize} we examine how the amount of sampled itinerary points affects the success rate of \ac{tshix}. In Section~\ref{sec:feedForward} we analyse the trajectory following performance of the controller and whether involving the dynamics from Section~\ref{sec:dynamics} in a 2D task improves the performance. Finally, in Section~\ref{sec:3Dsearch} we study the method with the 3D plug-and-socket task, and in Section~\ref{sec:discussion} we discuss the results.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/kuka_setup_pih_num.png}
        \caption{\small{Peg-in-Hole setup: 1) KUKA LWR4+, 2) \ac{ftsensor}, 3) Peg tool, 4) Cylinder with hole}}
        \label{fig:expSetupPih}
    \end{subfigure}
    ~           \begin{subfigure}[t]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/kuka_setup_plug_num.png}
        \caption{\small{The plug and socket setup: 1) KUKA LWR4+, 2) Grab-handle for users to manipulate the robot, 3) \ac{ftsensor}, 4) Plug tool, 5) Socket}}
        \label{fig:expSetupPlug}
    \end{subfigure}
    \caption{\small{The setups used for the experiments.}}\label{fig:expSetup}
\end{figure}

\subsection{Comparison Between Ergodic Control and \ac{tshix}}
\label{sec:tspVsErgodic}
We used the 2D peg-in-hole task (Fig.~\ref{fig:expSetupPih}) to compare the sampling based \ac{tshix} and ergodic control approaches for trajectory creation\footnote{To generate ergodic control trajectories we used the 
following open source implementation 
\url{https://github.com/dressel/ErgodicControl.jl}}. We first learned the 
exploratory distribution and
the dynamics from a single demonstration. 
Since the peg-in-hole task is conducted in the 2D plane on top of 
a cylinder, the orientation of the peg tool was fixed during both demonstration 
and reproduction. With \ac{tshix} we generated 30 different trajectories in the 
x-y-plane, each consisting of 300 points sampled from the learned exploration 
distribution. With the ergodic control we generated a trajectory that was approximately the same length as the mean of the \ac{tshix} trajectories. Finally, for trajectories 
provided by both algorithms we used the learned dynamics model to compute the 
superposed forces. 
 
We performed the comparison by randomly choosing 30 starting positions from within a circle of ca.~3~cm diameter, located roughly halfway between the originally demonstrated starting position  and the hole of the cylinder. The reason for moving the starting positions closer to the hole is that the demonstration acts as a worst case scenario, \ie the one end of the exploration distribution will be approximately at the starting position. The same exploratory distribution and dynamics were used for both algorithms. For \ac{tshix} we used a different randomly chosen trajectory with each starting position to average the inherent randomness, whereas for the ergodic control we used the same trajectory with each position, due to its deterministic nature. As this task does not involve rotations, the control was performed by feeding the trajectory and superposed forces to~\eqref{eq:impedanceControlForce}.

The results of the experiment can be seen in Table~\ref{tab:resultTspVsErgodic}. They show that \ac{tshix} performed 
slightly better than the ergodic control. In the five trials where \ac{tshix} failed, the ergodic control failed as well. 
These failures of both algorithms seemed to occur because the starting positions were too far away from the goal, as 
neither trajectory lead close enough to the hole. In the five trials where \ac{tshix} succeeded and ergodic control failed, 
the ergodic trajectory would usually go within the vicinity of the hole, but not cover it. This implies that the difference 
between the algorithms could stem from density of coverage. 

\begin{table}[h]
    \centering
    \begin{tabular}{l c c}
        \toprule
        Algorithm & Ergodic & \ac{tshix}\\
        \midrule
        Success rate & 20/30 & 25/30 \\
        Success percentage & 67\% & 83\% \\
        \bottomrule
    \end{tabular}
    \caption{\small{Success rates from peg-in-hole experiments from the two trajectory creation methods.}}
    \label{tab:resultTspVsErgodic}
\end{table}

One advantage of using the sampling-based \ac{tshix} is the flexibility in generating the trajectory. If a generated 
trajectory was unsuccessful or undesirable for other reasons, a new trajectory can easily be generated by changing the 
random seed for the sampling. Moreover, additional points could even be sampled during reproduction should the task fail. This is 
not possible for the ergodic trajectory, as they are per definition deterministic and thus when the chosen convergence 
criteria are met, the trajectory is finished. However, the ergodic trajectory can be considered optimal for covering a 
distribution~\cite{dressel2018optimality} and the deterministic nature increases the predictability and repeatability of 
the algorithm.

\subsection{Effect of Sample Size}
\label{sec:samplingSize}
To investigate the effect the sample size had on the success rate of \ac{tshix}, one successful starting position from 
previous section was selected for further analysis. We generated 20 trajectories for sample sizes of 100, 200, 300, 400 and 
500 each. More samples will lead to a higher coverage (see Fig.~\ref{fig:PiH_samp}) and the connection between coverage and 
success rate is investigated in this section. The trajectories and their corresponding predicted superposed forces were 
executed with the impedance controller from~\eqref{eq:impedanceControlForce}. The results, which can be seen in 
Table~\ref{tab:samplingSizeComp}, show that initially the success of the search increases with higher sample sizes. 
However, after 300 samples the success rate consistently stays at 85\%. It was thus determined that 300 sample points is a 
reasonable number to use for the peg-in-hole task. For a different task, the number would of course vary. However, a key 
observation is that after sufficient sample density, sampling more points does not increase the performance. 

\begin{table}[h]
    \centering
    \begin{tabular}{l c c c c c}
        \toprule
        Sample size & 100 & 200 & 300 & 400 & 500 \\
        \midrule
        Success rate & 6/20 & 12/20 & 17/20 & 17/20 & 17/20 \\
        Success percentage & 30\% & 60\% & 85\% & 85\% & 85\% \\
                \bottomrule
    \end{tabular}
    \caption{\small{Success rates from varying the number of sampled points in \ac{tshix} on the 2D peg-in-hole task }}
    \label{tab:samplingSizeComp}
\end{table}

\begin{figure}
    \centering
    \begin{subfigure}[tbp]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/PiH_samp100.pdf}
   		\caption{\small{100 samples}}
    		\label{fig:PiH_samp100}
    \end{subfigure}
    ~           \begin{subfigure}[tbp]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/PiH_samp500.pdf}
   		\caption{\small{500 samples}}
    		\label{fig:PiH_samp500}
    \end{subfigure}
   	\caption{\small{Different number of sampled points covering the learned exploration distribution.}} \label{fig:PiH_samp}
\end{figure}


\subsection{Controller Analysis}
\label{sec:feedForward}
For in-contact tasks it is a challenge to choose the right stiffness value such that the trajectory is followed while allowing compliance to avoid excessive contact forces and facilitate easier completion of the task. For peg-in-hole tasks, lower stiffness perpendicular to the motion allows the peg to be inserted without moving over the exact center of the hole, but taking advantage of the mechanical gradients of the task. 

Our choice was to keep the stiffness low and instead provide the robot with the dynamics of the task. The difference between knowing the dynamics and increasing the stiffness is that by knowing the dynamics, we can predict the forces necessary to counter the environmental forces, such as friction, along the trajectory. Thus the stiffness is increased only in the direction of motion while leaving the tool compliant perpendicular to the direction of motion. We empirically observed that this perpendicular compliance indeed seemed to play a key role in the final stage of the task where the peg has to slide into the hole; without the compliance the peg was more likely to slide by close to the hole but not sink in.

To experimentally examine how much influence the usage of the superposed forces has on the outcome of the task, an additional experiment series was set up. 20 trajectories from 100, 200 and 400 sampled points were created. Each trajectory was then executed with the impedance controller in Section~\ref{sec:samplingSize} without the addition of the superposed predicted forces. For the 100 sample point trajectories, only 2/20 trials succeeded, 4 less then with force-feed-forward. Similar observations were made for 200 and 400 sample point trajectories (7/20 and 13/20 respectively). This consistently inferior performance is indicative of the importance of the superposed forces even on a task performed on a 2D plane. As the forces are expected to be countering the environmental forces, which in this task consist of mainly friction, the forces point in the direction of the state change. 
This can be observed from Fig.~\ref{fig:PiH_predictedFrc} where the superposed forces are plotted over a trajectory sliding 
along 2D plane. We note that in this example the forces pointing "north-west" have smaller magnitude, and are thus more 
difficult to observe in the figure. 

\begin{figure}
    \centering
        \includegraphics[width = \columnwidth]{picture/experiments/PiH_predictedFrc_negated.pdf}
   		\caption{\small{The superposed forces calculated from learned dynamics plotted along a generated search trajectory.}}
    		\label{fig:PiH_predictedFrc}
\end{figure}


However, even with the superposed forces the tool is not following the desired trajectory accurately, as can be seen in Fig.~\ref{fig:PiH_comp}. These trajectories were completed with stiffness values that were experimentally found to provide a good balance between trajectory following and compliance that facilitates the final insertion of the peg-in-hole task. The reason for this divergence lies presumably in the unknown friction forces of the robot's joints. When performing the demonstrations, the teachers also noticed that the joint configuration had a significant effect on the ease of moving the robot. In addition, feeding a Cartesian wrench profile recorded from a demonstration to the robot in pure force control did not produce any meaningful results. We assume this is due to static friction in the joints that prevents initiation of small motions.


\begin{figure}
    \centering
    \begin{subfigure}[tbp]{0.45\columnwidth}
	\includegraphics[width = \columnwidth]{picture/experiments/PiH_comp_tsp.pdf}
   		\caption{}    		\label{fig:PiH_TSP_comp}
    \end{subfigure}
    ~           \begin{subfigure}[tbp]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/PiH_comp_erg.pdf}
   		\caption{}    		\label{fig:PiH_ERG_comp}
    \end{subfigure}
   	\caption{\small{Trajectory following performance of the controller on trajectories created by \ac{tshix} (a) and ergodic control (b).} \label{fig:PiH_comp}}
\end{figure}

\subsection{Learning a 3D Search Task}
\label{sec:3Dsearch}
In order to see how well the proposed method scales to higher dimensions, we created an experimental setup that requires a 
three-dimensional search to succeed. The task in question is to insert an electrical plug (Europlug) into a socket. For the 
socket, a 12V socket usually found in caravans and sheds was used because of its design: one hole is slightly larger, and 
there are valley shaped indentations around the holes, allowing an easier insertion when motion is compliant. To make the 
demonstrations and the learning process easier, the rotation around the x- and y-axes of the tool are restricted, so that 
the search was only performed in the positional space of the x-y-plane, as well as in rotation around the tool's z-axis. 
The demonstrations were conducted with closed eyes, and the starting pose of the plug was inside the socket close to a 
side wall. Additionally, the orientation around the z-axis was chosen randomly, but still reasonable enough to allow the 
teacher to complete the task like an everyday situation. Because of the higher complexity of this 3D task, we compared 
learning the exploration distribution from either one or two demonstrations. The two demonstrations were performed at 
opposite ends of the upper half of the socket (see Fig.~\ref{fig:plug_demo_start}). From both a single demonstration and a 
combination of two demonstrations, the 3D exploration distribution (position in x and y, rotation around z) and the 6D task 
dynamics (position in x and y, rotation around z, forces in x and y, torques around z) were learned similarly to the 
peg-in-hole task, by fitting a single Gaussian distribution over the data. A trajectory was created by sampling 600 points, 
which was found to be a reasonable number for covering the 3D exploration distribution (see 
Fig.~\ref{fig:Plug_trajectory}). Subsequently the predicted interaction values from the environment (both forces and 
torques) for the given trajectory were calculated.

For the experiments 15 starting positions were randomly chosen in the northern hemisphere of the socket, and for each 
starting position a different trajectory was generated from both one and two demonstrations. It was impossibly to create an 
ergodic trajectory with \ac{pto} in 3D, since the algorithm gets easily trapped in a local minimum which restricts the 
length of the created trajectory. In order to provide a baseline for comparison, random walk trajectories were created 
using the method proposed by Abu-Dakka et al.~\cite{abu2014solving}. The results are presented in 
Table~\ref{tab:result3Dtask}. We can observe that for the 3D task having two demonstrations significantly increases the 
success rate and even for the much harder socket task the method achieve good results.

\begin{table}[h]
    \centering
    \begin{tabular}{l c c c}
        \toprule
        Algorithm & Random Walk & 1-demo-\ac{tshix} & 2-demo-\ac{tshix} \\
        \midrule
        Success rate & 0/15 & 3/15 & 10/15 \\
        Success percentage & 0\% & 20\% & 67\% \\
        \bottomrule
    \end{tabular}
    \caption{\small{Success rates from plug-in-socket experiments from random walk and \ac{tshix} with either one or two demonstrations.}}
    \label{tab:result3Dtask}
\end{table}

\begin{figure}
    \centering
        \includegraphics[width = \columnwidth]{picture/experiments/Plug_traj2.pdf}
   		\caption{\small{Illustration of 3D trajectory created from 600 sample points.}}
    		\label{fig:Plug_trajectory}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[tbp]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/plug_left.png}
   		\caption{\small{Plug left.}}
    		\label{fig:plug_left}
    \end{subfigure}
    ~           \begin{subfigure}[tbp]{0.45\columnwidth}
        \includegraphics[width = \columnwidth]{picture/experiments/plug_right.png}
   		\caption{\small{Plug right.}}
    		\label{fig:plug_right}
    \end{subfigure}
   	\caption{\small{Starting positions of two demonstrations used to learn the exploration distribution.}} \label{fig:plug_demo_start}
\end{figure}

\subsection{Discussion}
\label{sec:discussion}
Results show that the proposed method performs well if the demonstrations' starting positions cover the variability of the 
scenarios. However, some real world scenarios such as plug-and-socket for a European 230V AC socket are surprisingly 
difficult, such that also human teachers found it very hard to solve the task blindly. This indicates that some search problems may be infeasible in higher dimensions. On the other hand, if the 
demonstrated search is performed in a lower-dimensional subspace of a high dimensional state space, the proposed method 
will automatically perform the search in the lower dimensional space by virtue of employing the Gaussian linear model. 

We showed that while it is possible to use only one demonstration to learn a search if the task is sufficiently easy, for more complex tasks with higher dimensionality it is necessary to have more demonstrations in order to achieve a reasonable convergence region. Furthermore, a requirement for the demonstrations is that they need to be performed in worst case scenarios, so that they cover the variability of both exploration region and dynamics encountered in the task. 








==> Sections/intro_prel.tex <==
\section{INTRODUCTION}
\label{intro}
To succeed in peg-in-hole type assembly tasks with small clearance between workpieces, a robot's internal model of the world must match with the environment to high precision, as even small errors in the model can cause the robot to fail.
In such events it is possible to rely on handcrafted exception strategies to complete the task, but the process of defining the strategies is tedious and error-prone.
Moreover, a human operator is often required to correct the model when an error occurs.
Our key insight is to make the robot behave similarly as a human would when faced with such uncertainties about the environment.
A natural human behaviour in such situations is to probe the environment, much like fitting a key into a lock in darkness or inserting a plug into an electric socket, as illustrated in Fig.~\ref{fig:plug_insertion}.
With this in mind, we present a \ac{lfd} method for teaching robots to perform human inspired search strategies.

    \begin{figure}
        \centering
        \begin{subfigure}[b]{0.225\textwidth}
            \centering
            \includegraphics[width=\textwidth]{picture/plug_1.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.225\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{picture/plug_2.png}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.225\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{picture/plug_3.png}
        \end{subfigure}
        \quad
        \begin{subfigure}[b]{0.225\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{picture/plug_4.png}
        \end{subfigure}
        \caption{\small An example sequence of a robot inserting a plug into a socket without vision sensing.} 
        \label{fig:plug_insertion}
    \end{figure}


In \ac{lfd} a human teacher performs one or more demonstrations that the robot 
then learns to mimic \cite{argall2009survey}. Methods to encode and 
parametrize the demonstrated skill are usually based on attractors along a 
trajectory, such as \ac{dmp} \cite{schaal2006dynamic} and \ac{gmm} with 
\ac{gmr} \cite{calinon2007learning}. However, these methods assume that the 
goal pose is either known or can be learned. In contrast, we target scenarios 
where the goal pose can vary between reproductions of the same task and cannot 
be visually identified with sufficient accuracy to complete the task. 







Optimizing a skill with a goal in an unknown location is often performed with \ac{rl} where the skill is learned by continuously interacting with the environment \cite{kober2012reinforcement}. Although \ac{rl} can learn complex assembly skills that can generalize to new situations \cite{levine2015learning}, the employed methods are data intensive, require handcrafted reward functions and much interaction with the environment before successfully learning the task. Such methods are therefore usually too time-consuming to employ in real on-line settings, a limitation our method addresses by learning successful search strategies from few human demonstrations.


We propose a method to learn search strategies by imitating human behaviour. Our proposed method consists of four steps: 1) gathering one or more human demonstrations from which forces and positions are recorded; 2) modelling the covered search area---termed \textit{exploration distribution}---and state-invariant dynamics of the task at hand; 3) planning a search trajectory over the exploration distribution; and 4) executing the search trajectory with an impedance controller while superimposing forces learned from dynamics. For planning the search trajectory we compare two algorithms: ergodic control approach proposed by Miller et al.~\cite{miller2013trajectory} and our own sampling-based algorithm \ac{tshix}. We evaluate our method in both 2D (peg-in-hole with a round peg) and 3D (inserting an electric plug into a socket) search tasks.


The main contributions in this work include 1) a novel 4-step framework  for learning search strategies including both position and force component from human demonstrations 2) a sampling based method, \ac{tshix}, for creating trajectories from an exploration distribution and 3) showing through experiments that our learned search strategies are suitable to work as exception strategies in a 3D assembly task.










==> Sections/method_prel.tex <==
\section{METHOD}
\label{sec:METHOD}



Our proposed method is a 4-step framework to learn search strategies from human demonstration for assembly tasks.
The first step of our method is learning the exploration distribution and is presented in Section~\ref{sec:exploDist}. 
Since we are dealing with exception cases, this step also imposes requirements on the demonstrations. 
From the exploration distribution we need to create the search trajectory for the manipulator to follow. This second step is presented in Section~\ref{sec:trajectory}.
There we propose two different methods, namely our own sampling-based method \ac{tshix} and a deterministic ergodic control method.
Since we address in-contact tasks which might require searching in force domain as well, we also need to learn the dynamics of the demonstration as the third step.
This is shown in Section~\ref{sec:dynamics}.
Finally, the last step of our method, presented in Section~\ref{sec:searchPerform}, performs the learned strategy with an impedance controller. 





\subsection{Learning the Exploration Distribution}
\label{sec:exploDist}

We model the exploration distribution by fitting a single Gaussian distribution over the recorded states, using Maximum Likelihood Estimation:
\begin{equation}\label{eq:exploDist_Gauss}
    p_{e}(\mbm{s}) = \mathcal{N} (\mbm{s}|\mbm{\mu},\matr{\Sigma})\ ,
\end{equation}
\noindent for each state $\mbm{s} \in S$, where $S$ is the $D \times N$ matrix of all $N$ states recorded during one or more demonstrations and $D$ is the dimension of the task.
Parameters $\mbm{\mu}$ and $\matr{\Sigma}$ are the learned mean vector and covariance matrix. 

Learning an expressive exploration distribution is conditioned on the quality of the demonstrations.
As such, human teachers should use similar sensing modalities as the robot.
As this work did not use any vision system  for the robot, the teacher performed the search with closed eyes.
To perform the actual search, the end-effector was placed in the proximity of the goal in a manner that resembles possible failure scenario of the robot's task.
The teacher grabbed the robot with his eyes closed and searched with his own strategy for the goal.
If the search failed such that the end-effector ended up in a configuration from which success without vision was improbable, the demonstration was stopped and discarded.
Similarly, if the goal was found immediately, that demonstration was also discarded as it gives little to no information about the exploration.
Therefore, only demonstrations that provide individual search trajectories that cover the exploration area effectively were saved as they provide most information in terms of search area and force/torque profile.

As our proposed method is for use in environments where the location information can be erroneous, we regard the information conveyed by the recorded trajectory and forces as more important than the starting location of the search. Thus we set each search -- both demonstrated and learned -- into a common coordinate frame, which in this paper is called 
the \textit{search frame}. Furthermore we choose to align the demonstrations based on their origin, not the goal, even though in the world coordinate system they share the goal but not the origin.
With this choice we can better learn the \textit{search} strategy of the teacher in situations where localizing the tool 
w.r.t~to the world frame is impossible.
Now we can define that any trajectory generated in this work will also start at the origin of the search frame.
Thus the learned searches are independent of their location in the world frame.



\subsection{Creating the Search Trajectory}
\label{sec:trajectory}
Given the modelled exploration distribution, the next step is to create a search trajectory that covers the distribution.
For this, two methods were proposed: 1) our own stochastic sampling-based 
\ac{tshix} and 2) a deterministic method, ergodic control 
\cite{miller2013trajectory}. 

\subsubsection{Trajectory Sampling from Human-Inspired eXploration}
\label{sec:tsp}
The algorithm we propose, \ac{tshix}, samples points from the exploration distribution created in~\ref{sec:exploDist}, 
finds an approximation of the shortest itinerary through the sampled points and smooths it. 

Since we model the exploration distribution as a Gaussian, we sample from the distribution using Marsaglia's ziggurat method~\cite{marsaglia1984fast}. As sampling is the main concept of this algorithm, the sample density plays a major role in \ac{tshix}. Visualizations of 
sampling in 2D are presented in Fig.~\ref{fig:PiH_samp}.
Independent from the number of samples, an itinerary needs to be generated that visits each sample point. 
However, as finding the optimal solution is NP-hard, we use a Genetic Algorithm \footnote{The algorithm models the problem as \ac{tsp} and finds a short-as-possible itinerary: \url{https://se.mathworks.com/matlabcentral/fileexchange/21198-fixed-start-open-travelling-salesman-problem-genetic-algorithm}} to approximate the shortest itinerary through all sample points. The start of the itinerary is always set at the origin of the search frame in an effort to imitate the human search, which is defined to start at the origin.
To provide the robot with a smooth trajectory to follow, the calculated itinerary is smoothed with a Savitzky-Golay Filter \cite{savGolFilter}.
Fig.~\ref{fig:PiH_TSP_comp} illustrates the stages of creating a traversable trajectory for 
the tool: A series of sample points is generated, through which an itinerary is calculated, which in turn is smoothed to produce the final trajectory.



\subsubsection{Ergodic Control}
\label{sec:ergodic}
Ergodic control is a method for creating a trajectory such that at every step the time-averaged behaviour of the system tries to match an underlying, known probability distribution.
In our case the underlying distribution is the exploration distribution we learn from the human demonstration in~\ref{sec:exploDist}.
Miller and Murphey~\cite{miller2013trajectory} showed that ergodic control can create trajectories that effectively covers probability distributions, and we will use their work as comparison.
Specifically, we will follow the methods from~\cite{miller2013trajectory}, which consists of 1) a metric for ergodicity from~\cite{mathew2011metrics} and 2) a control strategy called \ac{pto} \cite{hauser2002projection}.


\subsection{Learning the Task Dynamics}
\label{sec:dynamics}
From observing humans performing search tasks it can be inferred that they do not simply follow a trajectory in space, but maintain contact between the workpieces and deduce vicinity of alignment based on the contact forces.
Thus learning the dynamics is useful already for simple 2D cases, where it can be used to efficiently overcome the observed 
friction. In more complex problems where certain threshold forces are required to accomplish alignment, such as tasks 
requiring "snapping" \cite{stolt2011force}, using the forces is required. 
Thus, learning search strategies similar to humans requires not only to learn the explored states, but also the contact dynamics of how a human interacts with the environment during the search.

For this reason, a \ac{ftsensor} is attached to the wrist of 
the manipulator to record the contact forces during a demonstration.
More specifically, the forces and torques recorded by the \ac{ftsensor} at constant speed are sum of the normal force/torque 
and the friction cause by the motion.
Thus the direction of the measured forces is always opposing the direction of the demonstrated motions.

Additionally, if the states are considered points on a trajectory, the learned dynamics will be very specific to the location in the search frame.
This is undesirable since we do not assume to know the transformation from search frame to world frame, and thus such 
high-precision dynamics would not be applied correctly.
In order to avoid this and have the dynamics apply independent of the robots location in the demonstrated environment, the states are rendered location invariant. 

To compute the location invariant dynamics, a discrete set of points is sampled from the continuous trajectory function presented in Section~\ref{sec:trajectory}.
From the discrete set of points, the location invariant data is created by taking the difference between consecutive sampled points.
The resulting matrix, which we call $\Delta S$, is a $D \times (N-1)$ matrix. Each column $\Delta \mbm{s}_{t}$, where $t \in [1..N-1]$, is calculated by:

\begin{equation}\label{eq:locInvariance}
    \Delta \mbm{s}_{t} = \mbm{s}_{t+1} - \mbm{s}_{t}.
\end{equation}

We call the concatenation of the $1 \times D$ force vector $\mbm{f}_{t}$ and the $1 \times D$ torque vector $\mbm{t}_{t}$ at time $t \in [1..N-1]$ an \textit{action}, which is stored in the column vector $\mbm{a}_{t}$ such that
\begin{equation}
\mbm{a}_{t} = \left[ -\mbm{f}_{t},\ -\mbm{t}_{t} \right]^T,
\end{equation}
\noindent where the signs of $\mbm{f}_{t}$ and $\mbm{t}_{t}$ are reversed due to the need of creating feed-forward forces that overcome the measured forces.
Now given $\Delta \mbm{s}_{t}$ and $\mbm{a}_{t}$ recorded during a demonstration, we model the dynamics as a single Gaussian distribution.
Similarly to the exploration distribution, the dynamics model is fitted by using Maximum Likelihood Estimation.
This results in the following dynamics model
\begin{equation}\label{eq:multivarGauss_locInv}
    p_{d}(\Delta \mbm{s}, \mbm{a}) = \mathcal{N} (\Delta \mbm{s}, \mbm{a} | \mbm{\mu},\matr{\Sigma})\ ,
\end{equation}
\noindent where $\mbm{\mu}$ and $\matr{\Sigma}$ represent, respectively, the mean vector and covariance matrix of the dynamics distribution.


Once the task dynamics are learned, we can predict the interaction forces by conditioning the Gaussian distribution in~\eqref{eq:multivarGauss_locInv} on state changes.
To do this, first the mean vector $\mbm{\mu}$ in \eqref{eq:multivarGauss_locInv} is partitioned as follows:

\begin{equation}\label{eq:conditionalGauss2}
\mbm{\mu} = \left[ \mbm{\mu_{a}}\,\ \mbm{\mu_{s}} \right]^T ,
\end{equation}
\noindent where $\mbm{\mu_{a}}$ is the $D$-dimensional mean vector of the recorded actions and $\mbm{\mu_{s}}$ the $D$-dimensional mean vector of the recorded states.
The covariance matrix $\matr{\Sigma}$ in~\eqref{eq:multivarGauss_locInv} is partitioned into:

\begin{equation}\label{eq:conditionalGauss3}
\matr{\Sigma} = \begin{bmatrix}
\matr{\Sigma_{aa}} & \matr{\Sigma_{as}}\\
\matr{\Sigma_{sa}} & \matr{\Sigma_{ss}}
\end{bmatrix}\ ,
\end{equation}
\noindent where $\matr{\Sigma_{aa}},\matr{\Sigma_{as}},\matr{\Sigma_{sa}}$ and $\matr{\Sigma_{ss}}$ are $D \times D$ dimensional covariance matrices.

Given (\ref{eq:conditionalGauss2}-\ref{eq:conditionalGauss3}), we estimate the predicted action $\mbm{a}^*$ at each state by conditioning the dynamics model in~\eqref{eq:multivarGauss_locInv} on a location invariant state change $\Delta \mbm{s}^*$ computed from~\eqref{eq:locInvariance}:

\begin{equation}\label{eq:conditionalGauss4}
    ( \mbm{a}^*\ |\ \Delta \mbm{s}^* ) \sim \mathcal{N} (\mbm{\mu^*}, \matr{\Sigma^*})\ ,
\end{equation}

\noindent where

\begin{equation}\label{eq:conditionalGauss5}
    \mbm{\mu}^* = \mbm{\mu_{a}} + \matr{\Sigma_{as}} \matr{\Sigma_{ss}^{-1}}(\Delta \mbm{s}^* - \mbm{\mu_{s}})\ ,
\end{equation}

\noindent and

\begin{equation}\label{eq:conditionalGauss6}
    \matr{\Sigma}^* = \matr{\Sigma_{aa}} - \matr{\Sigma_{as}} \matr{\Sigma_{ss}^{-1}} \matr{\Sigma_{sa}}\ .
\end{equation}

The interaction force $\mbm{a}^*$ is set as the mean $\mbm{\mu}^*$ of the conditional distribution.
To retrieve the predicted actions for a complete trajectory, (\ref{eq:conditionalGauss4}-\ref{eq:conditionalGauss6}) need to be calculated for each state change $\Delta \mbm{s}^*$ of the trajectory.
Once the search trajectory and corresponding actions are estimated, they are fed to an impedance controller (Section~\ref{sec:searchPerform}) for execution on the robot.

\subsection{Performing the Search}
\label{sec:searchPerform}
To reproduce the search motions, we use an impedance controller with superposed forces and torques.
In general, impedance control mimics a virtual spring attached to the wrist of a manipulator.
The controller \textit{stiffness} gives a measure of how stiff the spring is, \ie how much force and torque does it apply against possible physical obstacles on the trajectory.
In this work we superimpose the impedance controller with an additional Force-Torque feed-forward component as visualized in Fig.~\ref{fig:impedanceControl}.
The resulting impedance control law for translations is:

\begin{equation}\label{eq:impedanceControlForce}
   \mbm{f}_{c} =  K_{p} \mbm{e}_{p} + B_{p} \Dot{\mbm{e}}_{p} + \mbm{f}_{f}\ ,
\end{equation}

\noindent where $\mbm{f}_c$ is the resulting force commanded to the robot, $\mbm{e}_{p}$ is the positional error between current and desired position, $K_{p}$ is the positional stiffness coefficient describing what force is required to move by $1~\text{m}$, $\Dot{\mbm{e}}_{p}$ is the derivative of the positional error, and $B_{p}$ is the positional damping coefficient describing what force is used to dampen the motion.
The additional $\mbm{f}_{f}$ term is the superimposed feed-forward forces. 

The impedance control law for orientations is

\begin{equation}\label{eq:impedanceControlTorque}
    \mbm{t}_{c} =  K_{\theta} \mbm{e}_{\theta} + B_{\theta} \Dot{\mbm{e}}_{\theta} + \mbm{t}_{f}\ ,
\end{equation}

\noindent where $\mbm{t}_c$ is the resulting torque commanded to the robot, $\mbm{e}_{\theta}$ is the angular error between current and desired orientation, $K_{\theta}$ is the angular stiffness coefficient, describing what torque is required to rotate by $1~\text{rad}$, $\Dot{\mbm{e}}_{\theta}$ is the derivative of the angular error, and $B_{\theta}$ is the angular damping coefficient, describing what torque is used to dampen the motion.
The additional $\mbm{t}_{f}$ term is the superimposed feed-forward torques.

Using an impedance controller enables a robot to follow a trajectory in free space as well as in contact while being compliant to the environment.
Using the superposed feed-forward forces enables force based searching provided the teacher demonstrates such behaviour.


\begin{figure}
\begin{overpic}[width=1.0\columnwidth,tics=10]{picture/methods/impedanceController_6D.pdf}
    \put(31, 51.5){$K_{\theta}$}
    \put(33.5, 39){$\dot{e}_{\theta}$}
    \put(45, 39.5){$B_{\theta}$}
    \put(72, 53){$\mbm{t}_{c}$}
    \put(48, 58.25){$\mbm{t}_{f}$}
        
    \put(31, 16){$K_{p}$}
    \put(33.5, 27.5){$\dot{e}_{p}$}
    \put(45, 27.5){$B_{p}$}
    \put(71.5, 14){$\mbm{f}_{c}$}
    \put(47, 10){$\mbm{f}_{f}$}
\end{overpic}
\caption{\small{An impedance controller with F/T feed-forward is used to reproduce the search motions.}}
\label{fig:impedanceControl}
\end{figure}





==> Sections/related_prel.tex <==
\section{RELATED WORK}
\label{RELATED}




Existing work on search motions primarily focus on exception strategies on a 2D plane. Abu-Dakka et al.~\cite{abu2014solving} presented an exception strategy based on stochastic search for the case when a peg-in-hole task failed. However, their method did not use any task-specific information, which could improve the accuracy. Jasim et al.~\cite{jasim2014position} used an Archimedean spiral to more effectively cover the 2D search area. However, the spiral requires hand-crafting and is not applicable in higher dimensional search tasks such as inserting a plug into a socket. Baum et al.~\cite{baum2017opening} compared different physical exploration strategies in a 3D scenario. However, they did not directly try to learn the search strategies from human demonstrations. 

A similar idea of using human demonstrations to learn search strategies was previously explored by De Chambrier in \cite{de2016learning}. He targeted the same problem of learning to plug a socket, but assumed the location of the socket stayed the same, or that the transformation between two socket locations was known. That method used 150 demonstrations to train a \ac{pomdp} which, in short, learned a strategy that first localized itself in the environment with the help of physical barriers, and afterwards followed a similar trajectory to the socket. In comparison, our method focuses on cases with known approximate location of the goal, while the position or orientation of the goal can change from one demo to another in an unknown manner, requiring physical exploration for insertion. Moreover, our method does not require such an extensive amount of demonstrations.

In De Chambrier's work, the actual insertion was performed according to the work of Kronander \cite[Chapter 5]{kronander2015control}. He also had an underlying hand-crafted strategy based on contact transients, and only in case of jamming the human teacher intervened. In contrast, our method can learn the whole search process from humans in cases where the approximate location and orientation of the hole is known, but the accuracy of the environment model is not high enough to plan a direct insertion trajectory. In addition, our method learns from human demonstration a search strategy consisting of both position and force distributions, thus allowing also force-based searching. Furthermore, the presented method does not require hand-crafting transient behaviours, but they are implicitly learned from the demonstrations alone.








